Spatial Entropy as an Inductive Bias for Vision Transformers

Recent work on Vision Transformers (VTs) showed that introducing a local inductive bias in the VT architecture helps reducing the number of samples necessary for training. However, the architecture modifications lead to a loss of generality of the Transformer backbone, partially contradicting the push towards the development of uniform architectures, shared, e.g., by both the Computer Vision and the Natural Language Processing areas. In this work, we propose a different and complementary direction, in which a local bias is introduced using an auxiliary self-supervised task, performed jointly with standard supervised training. Specifically, we exploit the observation that the attention maps of VTs, when trained with self-supervision, can contain a semantic segmentation structure which does not spontaneously emerge when training is supervised. Thus, we explicitly encourage the emergence of this spatial clustering as a form of training regularization. In more detail, we exploit the assumption that, in a given image, objects usually correspond to few connected regions, and we propose a spatial formulation of the information entropy to quantify this object-based inductive bias. By minimizing the proposed spatial entropy, we include an additional self-supervised signal during training. Using extensive experiments, we show that the proposed regularization leads to equivalent or better results than other VT proposals which include a local bias by changing the basic Transformer architecture, and it can drastically boost the VT final accuracy when using small-medium training sets. The code is available at https://github.com/helia95/SAR.

==> tables/ablation_lambda.tex <==
\begin{table}[ht]
  \centering
  \caption{IN-100, 100 epochs training. Influence of the spatial entropy loss weight ($\lambda$).}
\begin{tabularx}{\columnwidth}{lXXXXXX}
    \toprule
      \boldmath${\lambda}$ & 0 & 0.1 & 0.05 & 0.01 & 0.005 & 0.001 \\
    \midrule
    \textbf{Top-1 Acc.} & 75.72 & 75.88 & 76.22 & \textbf{76.72} & 76.16 & 75.82 \\
    \bottomrule
    \end{tabularx}
  
  \label{tab:lambda-ablation}
\end{table}

==> tables/ade20k_pvt.tex <==
\begin{table}[t]
\vspace{2mm}
\setlength{\tabcolsep}{1.0pt}
\small
    \caption{Segmentation downstream task on the ADE20K dataset.}
    \label{tab:ade20k_pvt}
    \centering
    \begin{tabular}{ll}
        \toprule
        \textbf{Model} & \textbf{mIoU} \\ 
        \midrule
        PVT-Small~\citep{PVT} & 39.8 \\
        \rowcolor{Light} PVT-Small+SAR & \textbf{41.1} \posimprov{0.3} \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/albation_architecture.tex <==
\begin{table}[ht]
  \centering
  \caption{An analysis of the different components of SAR on IN-100 (100 epochs training).}
\begin{tabularx}{\columnwidth}{Xl}
    \toprule
     \textbf{Model} & \textbf{Top-1 Acc}  \\
    \midrule
        A: Baseline  & 74.22 \\
        B: A + no MSA skip connections & 74.64   \posimprov{0.42} \\
        C: B +  no LN & 75.72    \posimprov{1.5} \\
        D: C +  no MLP skip connections & 73.76    \negimprov{0.46} \\
        E: A + spatial entropy loss & 74.78 \posimprov{0.56} \\
        F: A + SAR  & 76.72     \posimprov{2.5} \\
        \bottomrule
    \end{tabularx}
  \label{tab:Ablation}
\end{table}

==> tables/curves_occlusion_figures.tex <==
\begin{wrapfigure}[17]{r}{4.3cm}
    \centering
    \caption{IN-1K,  test set accuracy with respect to the number of training epochs.}
    \includegraphics[width=\linewidth]{figures/epochs.pdf}
    \label{fig:curves}
\end{wrapfigure}

\begin{figure}[t]
    \begin{minipage}[t]{0.6\linewidth}
    \kern0pt
    \centering
    \setlength\tabcolsep{0.0pt}
    \renewcommand{\arraystretch}{0.0}
    \begin{tabular}{ccc}
         \scalebox{0.55}{ViT-S/16} & \scalebox{0.55}{CvT-13} & \scalebox{0.55}{ViT-S/16+SAR} \vspace{0.05em} \\
         \includegraphics[trim=2 0 0 2,clip,width=0.33\columnwidth]{figures/baseline_bear.png} &
         \includegraphics[trim=2 0 0 2,clip,width=0.33\columnwidth]{figures/cvt_bear.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.33\columnwidth]{figures/sar_bear.png}
    \end{tabular}
    \captionof{figure}{TODO}
    \label{fig:figure1}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.4\linewidth}
    \kern0pt
    \centering
    \includegraphics[width=0.85\columnwidth]{figures/epochs.pdf}
    \caption{IN-1K,  test set accuracy with respect to the number of training epochs.}
    \label{fig:curves}
    \end{minipage}
\end{figure}

==> tables/in100_results.tex <==
\begin{table}[ht]
  \centering
  \caption{Influence of the number of epochs  on IN-100.}
\begin{tabularx}{\columnwidth}{Xlll}
    \toprule
     \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{ImageNet-100}} \\ 
	\cmidrule(lr){2-3} 
    & 100 epochs & 300 epochs\\
    \midrule
    Baseline & 74.22 & 80.82\\
    \rowcolor{Light}Baseline + SAR &\textbf{76.72} \posimprov{2.5} & \textbf{85.24}  \posimprov{4.42} \\
    \bottomrule
    \end{tabularx}
  \label{tab:IN-100}
\end{table}

==> tables/in100_sampling_ratio.tex <==
\begin{table}[t]
\vspace{2mm}
\setlength{\tabcolsep}{1.0pt}
\small
\caption{IN-100 experiments with different sampling ratios.}
\label{tab:sampling_ratio_in100}
\centering
    \begin{tabular}{lll}
    \toprule
    \textbf{Sampling Ratio} & \textbf{ViT-S/16} & \textbf{ViT-S/16+SAR}\\ 
    \midrule
    0.25 & 21.66 &  \cellcolor{Light}29.06 \posimprov{7.4} \\
    0.50 & 29.86 &  \cellcolor{Light}38.02 \posimprov{8.16} \\
    0.75 & 35.62 &  \cellcolor{Light}46.12 \posimprov{10.5} \\
    1.00 & 74.22 &  \cellcolor{Light}76.72 \posimprov{2.5} \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/in1k_results.tex <==
\begin{table*}[ht]
  \small
  \setcounter{table}{1}
  \centering
  \caption{IN-1K experiments with different VTs. For each tested VT, we plugged SAR on the publicly available code of the corresponding baseline and we used the suggested hyperparameter values for training. All results but ours are reported from the corresponding paper indicated in the  column ``Training Protocol''. All the results have been obtained using 300 training epochs.}
  \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{lllll}
    \toprule
   \textbf{Architecture} & \textbf{Training Protocol} & \textbf{Params (M)} & \textbf{FLOPs (G)} & \textbf{Top-1 Acc.} \\
   \midrule
   ViT-T/16 & DEiT~\citep{DeiT}  & 5 & 1.6 & 72.2 \\
   \rowcolor{Light}ViT-T/16 + SAR  & DEiT~\citep{DeiT}  &  5 & 1.6 & \textbf{72.4} \posimprov{0.2} \\
   ViT-S/16 & DEiT~\citep{DeiT}  &  22 & 4.7 & 79.8 \\
   \rowcolor{Light}ViT-S/16 + SAR &  DEiT~\citep{DeiT} & 22  & 4.7 & \textbf{80.7} \posimprov{0.9} \\
%   ViT-B/16~\cite{ViT} & DEiT  & 86 & 17.6 & 81.8 \\
%   \rowcolor{Light}ViT-B/16 + SAR & DEiT  & 86 & 17.6 & TODO \\
   \midrule
   T2T-ViT-14 & T2T~\citep{T2T}  & 21.5 & 6.1 & 81.5 \\
   \rowcolor{Light}T2T-ViT-14 + SAR & T2T~\citep{T2T}  & 21.5 & 6.1 & \textbf{81.9} \posimprov{0.4} \\
   \midrule
   PVT-Small & PVT~\citep{PVT}  & 24.5 & 3.8 & 79.8 \\
   \rowcolor{Light}PVT-Small + SAR & PVT~\citep{PVT}  & 24.5 & 3.8 & 79.84 \posimprov{0.04} \\
   \midrule
    CvT-13 & CvT~\citep{CvT}  & 20 & 4.5 & 81.6 \\
   \rowcolor{Light}CvT-13 + SAR & CvT~\citep{CvT}  & 20 & 4.5 & \textbf{81.8} \posimprov{0.2}  \\
   \bottomrule
   \end{tabular}}
  \label{tab:ImageNet-1K}
  
\end{table*}

==> tables/medium_small_dataset_results.tex <==
% Uncomment for Single Table
% \begin{table}[h]
%     \centering
%     \caption{TODO}
%     \begin{minipage}
%     \end{minipage}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lllll|llll}
%     \toprule
%     \textbf{Method} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Flowers} & \textbf{Pets} & \textbf{Cars} & 
%     \textbf{Clipart} & \textbf{Painting} & \textbf{Sketch} \\\midrule
%     ViT-S/16 & 80.1  & 58.35 & 42.02 & 24.58 & 35.3  & 41.0 & 38.4 & 37.2 \\
%     \rowcolor{Light}ViT-S/16+SAR & 81.83 \posimprov{1.73} & 59.89 \posimprov{1.54} & 40.88 \negimprov{1.14}  & 25.29 \posimprov{0.71}  & 64.65 \posimprov{29.35} & 64.95 \posimprov{23.95} & 57.11 \posimprov{18.17}  & 62.98 \posimprov{30.78} \\
%     \bottomrule
%     \end{tabular}}
%     \label{tab:my_label}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Two tables side by side
% \begin{table}[h]
%     \setlength{\tabcolsep}{1.0pt}
%     \footnotesize
%     \begin{minipage}[t]{.5\textwidth}
%     %\kern0pt
%     \caption{TODO}
%     \centering
%         \resizebox{\columnwidth}{!}{
%         \begin{tabular}{lllll}
%         \toprule
%         \textbf{Method} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Flowers} & \textbf{Pets} \\
%         ViT-S/16 & 80.1  & 58.35 & 42.02 & 24.58 \\
%         \rowcolor{Light}ViT-S/16+SAR & 81.83 \posimprov{1.73} & 59.89 \posimprov{1.54} & 40.88 \negimprov{1.14}  & 25.29 \posimprov{0.71} \\
%         \bottomrule
%         \end{tabular}}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{.5\textwidth}
%     %\kern0pt
%     \centering
%     \caption{TODO}
%         \resizebox{\columnwidth}{!}{
%         \begin{tabular}{lllll}
%         \toprule
%         \textbf{Method} & \textbf{Cars} & \textbf{Clipart} & \textbf{Painting} & \textbf{Sketch} \\
%         ViT-S/16 & 35.3  & 41.0 & 38.4 & 37.2  \\
%         \rowcolor{Light}ViT-S/16+SAR & 64.65 \posimprov{29.35} & 64.95 \posimprov{23.95} & 57.11 \posimprov{18.17}  & 62.98 \posimprov{30.78} \\
%         \bottomrule
%         \end{tabular}}
%     \end{minipage}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%
% Two tables side by side - improvement below

% \begin{table}[h]
%     \setlength{\tabcolsep}{1.0pt}
%     \footnotesize
%     \caption{Training from scratch on small-medium datasets.}
%     \centering
%     \begin{tabular}{lcccccccc}
%         \toprule
%         \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{(a)} & \multicolumn{4}{c}{(b)} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%         & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Flowers} & \textbf{Pets} & \textbf{Cars} & \textbf{Clipart} & \textbf{Painting} & \textbf{Sketch}  \\ \midrule   
%         ViT-S/16 & 80.1  & 58.35 & \textbf{42.02} & 24.58 & 35.3  & 41.0 & 38.4 & 37.2  \\
%         \rowcolor{Light}ViT-S/16+SAR & \textbf{81.83} & \textbf{59.89} & 40.88 & \textbf{25.29} & \textbf{64.65} & \textbf{64.95} & \textbf{57.11} & \textbf{62.98} \\
%         \rowcolor{Light} & \posimprov{1.73} & \posimprov{1.54} & \negimprov{1.14} & \posimprov{0.71} & \posimprov{29.35} & \posimprov{23.95} & \posimprov{18.17}  &   \posimprov{30.78}\\ 
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[h]
\small
    \centering
    \caption{Training from scratch on small-medium datasets.}
    \begin{tabular}{lllll}
    \toprule
        \textbf{Model} & \textbf{Cars} & \textbf{Clipart} & \textbf{Painting} & \textbf{Sketch} \\
        \midrule
        ViT-S/16 & 35.3  & 41.0 & 38.4 & 37.2  \\
        \rowcolor{Light}ViT-S/16+SAR & \textbf{64.65} \posimprov{29.35} & \textbf{64.95} \posimprov{23.95} & \textbf{57.11} \posimprov{18.17} & \textbf{62.98} \posimprov{30.78}\\
        \bottomrule
    \end{tabular}
    \label{tab:medium_size_dataset}
\end{table}





%\begin{table}[h]
%    \setlength{\tabcolsep}{1.0pt}
%    \footnotesize
%    \begin{minipage}[t]{.5\textwidth}
%    %\kern0pt
%    \caption{TODO}
%    \centering
%        \resizebox{\columnwidth}{!}{
%        \begin{tabular}{lcccc}
%        \toprule
%        \textbf{Method} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Flowers} & \textbf{Pets} \\
%        ViT-S/16 & 80.1  & 58.35 & \textbf{42.02} & 24.58 & 35.3  & 41.0 & 38.4 & 37.2  \\
%        \rowcolor{Light}ViT-S/16+SAR & \textbf{81.83} & \textbf{59.89} & 40.88 & \textbf{25.29} \\
%        \rowcolor{Light} & \posimprov{1.73} & \posimprov{1.54} & \negimprov{1.14} & \posimprov{0.71} \\ 
%        \bottomrule
%        \end{tabular}}
%    \end{minipage}
%    \hfill
%    \begin{minipage}[t]{.5\textwidth}
%    %\kern0pt
%    \centering
%    \caption{TODO}
%        \resizebox{0.90\columnwidth}{!}{
%        \begin{tabular}{lcccc}
%        \toprule
%        \textbf{Method} & \textbf{Cars} & \textbf{Clipart} & \textbf{Painting} & \textbf{Sketch} \\
%        ViT-S/16 & 35.3  & 41.0 & 38.4 & 37.2  \\
%        \rowcolor{Light}ViT-S/16+SAR & \textbf{64.65} & \textbf{64.95} & \textbf{57.11} & \textbf{62.98} \\
%        \rowcolor{Light} & \posimprov{29.35} & \posimprov{23.95} & \posimprov{18.17}  &   \posimprov{30.78} \\ 
%        \bottomrule
%        \end{tabular}}
%    \end{minipage}
%\end{table}

==> tables/pascal_results.tex <==
\begin{table}
  \centering
  \caption{A  comparison of the segmentation properties of the attention maps (PASCAL VOC-12).}
    \begin{tabularx}{0.85\columnwidth}{Xl}
    \toprule
     \textbf{Method} & \textbf{Jaccard similarity}  \\
    \midrule
        ViT-S/16  & 19.18 \\
        \rowcolor{Light}ViT-S/16 + SAR  & 31.19  \posimprov{12.01} \\
        \bottomrule
    \end{tabularx}
  
  \label{tab:PASCAL-VOC}
\end{table}


% \begin{wraptable}[6]{r}{5cm}
%     \vspace{-5mm}
%     \caption{A  comparison of the segmentation properties of the attention maps (PASCAL VOC-12).}
%     \label{tab:PASCAL-VOC}
%     \resizebox{\linewidth}{!}{
%     \begin{tabularx}{0.45\columnwidth}{Xl}
%     \toprule
%      \textbf{Method} & \textbf{Jaccard similarity}  \\
%     \midrule
%         ViT-S/16  & 19.18 \\
%         \rowcolor{Light}ViT-S/16+SAR  & 31.19  \posimprov{12.01} \\
%         \bottomrule
%     \end{tabularx}}
% \end{wraptable}

==> tables/pascal_robustness_results.tex <==
% \begin{table}[t]
% \vspace{2mm}
% \setlength{\tabcolsep}{1.0pt}
% \caption{(a) Out-of-distribution testing robustness. (b) A  comparison of the segmentation properties of the attention maps on PASCAL VOC-12. }
% \label{tab:robustness_results}
% \label{tab:PASCAL-VOC}
% \small
%     \begin{minipage}[b]{.59\textwidth}
%     \captionsetup{labelformat=empty} 
%     \centering
%     \begin{tabular}{lll}
%     % \footnotesize
%     \toprule
%     \textbf{Model} &  \textbf{ImageNet-A} (Acc. $\uparrow$)  & \textbf{ImageNet-C} (mCE $\downarrow$)\\ %{\em lower is better})\\
%     \midrule
%     ViT-S/16  & 19.2  & 52.8  \\
%     \rowcolor{Light}ViT-S/16+SAR & \textbf{22.39} \posimprov{3.19} & \textbf{51.6} \negimprovgreen{1.2} \\
%     %\posimprov{3.19}
%     \bottomrule 
%     \end{tabular}
%     \vspace{1.0mm}
%     \caption{(a)}
    
%     %\kern0pt
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{.4\textwidth}
%     \captionsetup{labelformat=empty} 
%     \centering
%         \begin{tabular}{ll}
%         \toprule
%         \textbf{Model} & \textbf{Jaccard similarity} ($\uparrow$)  \\
%         \midrule
%         ViT-S/16  & 19.18 \\
%         \rowcolor{Light}ViT-S/16+SAR  & \textbf{31.19}  \posimprov{12.01} \\
%         \bottomrule
%         \end{tabular}
%     \vspace{1.0mm}
%     \caption{(b)}
    
%     %\kern0pt
%     \end{minipage}
% %\vspace{-3mm}
% \end{table}

\begin{table*}[t]
\setlength{\tabcolsep}{1.0pt}
%\caption{(a) Out-of-distribution testing robustness. (b) A  comparison of the segmentation properties of the attention maps on PASCAL VOC-12. }
%\label{tab:robustness_results}
%\label{tab:PASCAL-VOC}
\small
    \begin{minipage}[b]{.48\textwidth}
    \caption{Out-of-distribution testing  on ImageNet-A (IN-A) and ImageNet-C (IN-C).}
    \label{tab:robustness_results}
    \centering
    \begin{tabularx}{\linewidth}{Xll}
    % \footnotesize
    \toprule
    \textbf{Model} &  \textbf{IN-A} (Acc. $\uparrow$)  & \textbf{IN-C} (mCE $\downarrow$)\\ %{\em lower is better})\\
    \midrule
    ViT-S/16  & 19.2  & 52.8  \\
    \rowcolor{Light}ViT-S/16 + SAR & \textbf{22.39} \posimprov{3.19} & \textbf{51.6} \negimprovgreen{1.2} \\
    %\posimprov{3.19}
    \bottomrule 
    \end{tabularx}
    %\caption{(a)}
    %\kern0pt
    \end{minipage}
    \hfill
    \begin{minipage}[b]{.49\textwidth}
    %\captionsetup{labelformat=empty} 
    \caption{A  comparison of the segmentation properties of the attention maps on PASCAL VOC-12.}
    \label{tab:PASCAL-VOC}
    \centering
        \begin{tabularx}{\linewidth}{Xll}
        \toprule
        \textbf{Model} & \textbf{Jaccard similarity} ($\uparrow$)  \\
        \midrule
        ViT-S/16  & 19.18 \\
        \rowcolor{Light}ViT-S/16 + SAR  & \textbf{31.19}  \posimprov{12.01} \\
        \bottomrule
        \end{tabularx}
    %\caption{(b)}
    %\kern0pt
    \end{minipage}
\end{table*}

==> tables/robustness_results.tex <==
\begin{table}[h!]
    \centering
    \label{tab:time-memory}
    % \resizebox{0.4\textwidth}{!}{%
    \begin{tabular}{lcc}
    % \footnotesize
    \toprule
    Method &  ImageNet-A (Acc. $\uparrow$)  & ImageNet-C (mCE $\downarrow$)\\ %{\em lower is better})\\
    \midrule
    ViT-S/16  & 19.2  & 52.8  \\
    ViT-S/16+SAR & {\bf 22.39} & {\bf 51.6}   \\
     %                &  \posimprov{29.35} &  \posimprov{23.95} &  &  \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/small_datasets.tex <==
\begin{table}[h]
    \centering
    \caption{Training from scratch on very small datasets. \elia{Moved from main paper} \marco{how many epochs? Moreover, I do not remember what we decided about these, shall we include them?} \elia{100, no decison yet, I think we can also remove it.}}
    \small
    \begin{tabular}{lllll}
    \toprule 
    \textbf{Method} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Flowers} & \textbf{Pets} \\
    \midrule
    ViT-S/16 & 80.1  & 58.35 & \textbf{42.02} \posimprov{1.14} & 24.58 \\
    \rowcolor{Light}ViT-S/16+SAR & \textbf{81.83} \posimprov{1.73}& \textbf{59.89} \posimprov{1.54} & 40.88 & \textbf{25.29} \posimprov{0.71} \\
    \bottomrule
    \end{tabular}
    \label{tab:small_size_dataset}
\end{table}

==> tables/tab3_4.tex <==
\begin{table*}[t]
\vspace{2mm}
\setlength{\tabcolsep}{1.0pt}
%\caption{(a) Out-of-distribution testing robustness. (b) A  comparison of the segmentation properties of the attention maps on PASCAL VOC-12. }
%\label{tab:robustness_results}
%\label{tab:PASCAL-VOC}
\small
    \begin{minipage}[b]{.29\textwidth}
    \caption{Training from scratch on small-medium datasets.}
    \label{tab:medium_size_dataset}
    \centering
    % \begin{tabular}{lllll}
    % \toprule
    %     \textbf{Model} & \textbf{Cars} & \textbf{Clipart} & \textbf{Painting} & \textbf{Sketch} \\
    %     \midrule
    %     ViT-S/16 & 35.3  & 41.0 & 38.4 & 37.2  \\
    %     \rowcolor{Light}ViT-S/16+SAR & \textbf{64.65} \posimprov{29.35} & \textbf{64.95} \posimprov{23.95} & \textbf{57.11} \posimprov{18.17} & \textbf{62.98} \posimprov{30.78}\\
    %     \bottomrule
    % \end{tabular}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcl}
        \toprule
        \textbf{Model} &  \textbf{ViT-S/16} & \textbf{ViT-S/16+SAR} \\
        \midrule
        Cars & 35.3 & \cellcolor{Light}\textbf{64.65} \posimprov{29.35} \\
        Clipart & 41.0 & \cellcolor{Light}\textbf{64.95} \posimprov{23.95} \\
        Painting & 38.4 & \cellcolor{Light}\textbf{57.11} \posimprov{18.17} \\
        Sketch & 37.2 & \cellcolor{Light}\textbf{62.98} \posimprov{30.78}\\
        \bottomrule
    \end{tabular}}
    %\caption{(a)}
    %\kern0pt
    \end{minipage}
    \hfill
    \begin{minipage}[b]{.68\textwidth}
    %\captionsetup{labelformat=empty} 
    \caption{Transfer learning results.% on different datasetes (100 epochs fine-tuning). 
    The first row corresponds to a standard fine-tuning protocol, while  the other configurations include SAR either in the pre-training or in the fine-tuning stage.}
    \label{tab:fine-tuning}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccllll}
    \toprule
    \textbf{SAR pre-training} & \textbf{SAR fine-tuning} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Flowers} & \textbf{Pets} \\
    \midrule
    \xmark & \xmark & 98.59 & 88.95 & 95.07 & 92.21 \\
    \rowcolor{Light}     \cmark   & \xmark & 98.69 \posimprov{0.1} & 89.19 \posimprov{0.24} & 96.05 \posimprov{0.98} & 92.7 \posimprov{0.49} \\
    \rowcolor{Light} \xmark & \cmark & 98.72 \posimprov{0.13} & 88.95 & 95.1 \posimprov{0.03}  & 92.34 \posimprov{0.13} \\
    \rowcolor{Light} \cmark & \cmark & 98.65 \posimprov{0.06} & 89.21 \posimprov{0.26} & 96.1 \posimprov{1.03} & 92.7 \posimprov{0.49} \\
    \bottomrule
    \end{tabular}}
    %\caption{(b)}
    %\kern0pt
    \end{minipage}
    \vspace{-3mm}
\end{table*}


==> tables/transfer_learning_results.tex <==
\begin{table*}[!ht]
\small
  \centering
  \caption{Transfer learning results on different datasetes (100 epochs fine-tuning). The first row corresponds to a standard fine-tuning protocol, while  the other configurations include SAR either in the pre-training or in the fine-tuning stage.}
  %\resizebox{0.7\linewidth}{!}{
    \begin{tabular}{ccllll}
    \toprule
    \textbf{SAR pre-training} & \textbf{SAR fine-tuning} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Flowers} & \textbf{Pets} \\
    \midrule
    \xmark & \xmark & 98.59 & 88.95 & 95.07 & 92.21 \\
    \rowcolor{Light}     \cmark   & \xmark & 98.69 \posimprov{0.1} & 89.19 \posimprov{0.24} & 96.05 \posimprov{0.98} & 92.7 \posimprov{0.49} \\
    \rowcolor{Light} \xmark & \cmark & 98.72 \posimprov{0.13} & 88.95 & 95.1 \posimprov{0.03}  & 92.34 \posimprov{0.13} \\
    \rowcolor{Light} \cmark & \cmark & 98.65 \posimprov{0.06} & 89.21 \posimprov{0.26} & 96.1 \posimprov{1.03} & 92.7 \posimprov{0.49} \\
    \bottomrule
    \end{tabular}%}
  \label{tab:fine-tuning}
\end{table*}
    
